CWEval: Outcome-driven Evaluation on Functionality and Security of LLM Code Generation

Large Language Models (LLMs) have significantly aided developers by generating or assisting in code writing, enhancing productivity across various tasks. While identifying incorrect code is often straightforward, detecting vulnerabilities in functionally correct code is more challenging, especially for developers with limited security knowledge, which poses considerable security risks of using LLM-generated code and underscores the need for robust evaluation benchmarks that assess both functional correctness and security. Current benchmarks like CyberSecEval and SecurityEval attempt to solve it but are hindered by unclear and impractical specifications, failing to assess both functionality and security accurately. To tackle these deficiencies, we introduce CWEval, a novel outcome-driven evaluation framework designed to enhance the evaluation of secure code generation by LLMs. This framework not only assesses code functionality but also its security simultaneously with high-quality task specifications and outcome-driven test oracles which provides high accuracy. Coupled with CWEval-bench, a multilingual, security-critical coding benchmark, CWEval provides a rigorous empirical security evaluation on LLM-generated code, overcoming previous benchmarks' shortcomings. Through our evaluations, CWEval reveals a notable portion of functional but insecure code produced by LLMs, and shows a serious inaccuracy of previous evaluations, ultimately contributing significantly to the field of secure code generation. We open-source our artifact at: https://github.com/Co1lin/CWEval .

==> sections/0_old_intro.tex <==
\begin{abstract}
\iffalse
Machine learning-based program synthesis, commonly known as code generation, have become prominent areas of research, providing developers with tools to generate functionally correct code from contextual inputs. 
However, these models can unintentionally produce vulnerable code, posing significant security risks if such code is unknowingly utilized, particularly by inexperienced programmers. 
This highlights the critical need to evaluate the security of code generation models. 
Current benchmarks for assessing the security of LLM-generated code often rely on third-party tools, such as CodeQL, and datasets that are limited to a small set of languages, such as Python, C, and C++.
These approaches can lead to incomplete assessments and false-positive evaluations. 
To address these limitations, we present \dataset, a robust, multi-language evaluation dataset specifically designed to evaluate the security of LLM-generated code. 
\dataset comprises PLACEHOLDER samples spanning PLACEHOLDER vulnerability types across PLACEHOLDER programming languages, all aligned with the Common Weakness Enumeration (CWE) standard. 
We demonstrate the utility of \dataset by applying it to evaluate PLACEHOLDER, offering valuable insights into the security capabilities of these models.
We released \dataset in our repository: PLACEHOLDER.
\fi




\end{abstract}

Machine learning-based program synthesis, or code generation, has emerged as a rapidly advancing field of research.
These models are used to assist software developers by generating functionally correct source code based on a given prompt, which can be natural language descriptions or partial code snippets in the form of comments or function signatures~\cite{allamanis2018survey}. 
Large-language Models (LLMs) use attention-based transformers~\cite{vaswani2017attention}, and are pre-trained with text data including code snippets from open-source platforms such as GitHub.
And they are later fine-tuned for code-related tasks such as code generation~\cite{sun2020treegen, svyatkovskiy2020intellicode}, code completion~\cite{svyatkovskiy2021fast, izadi2022codefill, kim2021code}, and code summarization~\cite{gao2022m2ts}.
By automating repetitive or complex coding tasks, code generation tools have the potential to significantly boost productivity and reduce development time. 
However, alongside their benefits, these models also pose potential risks, particularly when they generate insecure or vulnerable code~\cite{pearce2022asleep, siddiq2022empirical}. 
This is because they are trained on open-source code projects, which can consists security flaws~\cite{iannone2022secret, santos2017understanding, santos2019empirical}.
Such vulnerabilities can be particularly problematic if they go unnoticed by developers, especially those with limited experience in secure coding practices.

The unintentional generation of vulnerable code introduces a serious security threat, as it can lead to exploitable flaws in software systems. Vulnerabilities in automatically generated code may not only compromise individual applications but can also propagate systemic risks across dependent systems. For instance, if insecure code is integrated into production environments without proper vetting, it could expose organizations to attacks such as data breaches, privilege escalations, or denial-of-service incidents. The risks are exacerbated when these models are used by programmers who lack the expertise to identify and mitigate vulnerabilities.
Thus, it is essential to evaluate the output of these LLM based code generation models so that the generated code is not only functionally correct, but also is secure against vulnerability/insecure code.

Given these challenges, evaluating the security of code generation models is an essential task. 
Existing benchmarks for assessing the security of code generated by large language models (LLMs) rely heavily on static analysis tools, such as CodeQL, to detect vulnerabilities~\cite{siddiq2022securityeval, bhatt2024cyberseceval, bhatt2023purple}. While these tools provide a foundation for evaluation, their reliance on predefined patterns and heuristics can result in false positives and fail to capture nuanced or context-dependent security issues. Furthermore, most existing datasets used for benchmarking focus on a limited number of programming languages, such as Python and C, leaving other widely used languages underrepresented. This narrow scope restricts the generalizability of these evaluations and overlooks the diversity of real-world programming environments.

To address these limitations, we introduce \dataset, a comprehensive, multi-language dataset specifically designed to evaluate the security of code generated by LLMs. 
\dataset provides a diverse set of PLACEHOLDER samples, encompassing PLACEHOLDER vulnerability types across PLACEHOLDER programming languages, all aligned with the Common Weakness Enumeration (CWE) standard. 
This alignment ensures that the dataset is both systematic and aligned with widely recognized vulnerability taxonomies, making it suitable for evaluating a broad range of code generation scenarios. 
In addition, unlike existing benchmarks, \dataset use test cases based evaluation rather than relying on third-party tools such as CodeQL, providing a more holistic and robust evaluation framework.

In this paper, we demonstrate the utility of \dataset by applying it to evaluate PLACEHOLDER, comparing the performance of both open-source and closed-source code generation models. 
The results provide valuable insights into the strengths and weaknesses of these models in generating secure code, highlighting areas for improvement. 
By introducing \dataset, we aim to advance the field of secure code generation and provide a foundation for developing safer and more reliable code generation models.
We released this dataset in our repository: PLACEHOLDER.

